Improving the Bootstrap of Blind Equalizers with Variational Autoencoders

We evaluate the start-up of blind equalizers at critical working points, analyze the advantages and obstacles of commonly-used algorithms, and demonstrate how the recently-proposed variational autoencoder (VAE) based equalizers can improve bootstrapping.

==> chapters/acros.tex <==
\acrodef{AWGN}[AWGN]{additive white Gaussian noise}

\acrodef{BMI}[BMI]{binary mutual information}
\acrodef{BPS}[BPS]{blind phase search}

\acrodef{CD}[CD]{chromatic dispersion}
\acrodef{CMA}[CMA]{constant-modulus algorithm}
\acrodef{CNN}[CNN]{convolutional neural network}
\acrodef{CPE}[CPE]{carrier-phase estimation}

\acrodef{DFE}[DFE]{decision feedback equalizer}
\acrodef{DP}[DP]{dual-polarization}
\acrodef{DSP}[DSP]{digital signal processing}

\acrodef{ELU}[ELU]{exponential linear unit}
\acrodef{ELBO}[ELBO]{evidence lower bound}

\acrodef{FEC}[FEC]{forward error correction}
\acrodef{FIR}[FIR]{finite impulse response}

\acrodef{IP}[IR]{impulse response}
\acrodef{ISI}[ISI]{inter-symbol interference}

\acrodef{KL}[KL]{Kullback-Leibler}

\acrodef{LDPC}[LDPC]{low-density parity-check}
\acrodef{LLR}[LLR]{log-likelihood ratio}

\acrodef{MA}[MA]{moving average}
\acrodef{MAP}[MAP]{maximum a~posteriori}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{ML}[ML]{maximum likelihood}
\acrodef{MMA}[MMA]{multi-modulus algorithm}
\acrodef{MMSE}[MMSE]{minimum mean squared error}

\acrodef{NN}[NN]{neural network}

\acrodef{PCS}[PCS]{probabilistic constellation shaping}
\acrodef{pdf}[pdf]{probability density function}
\acrodef{PMD}[PMD]{polarization mode dispersion}
\acrodef{pmf}[pmf]{probability mass function}
\acrodef{PSK}[PSK]{phase shift keying}
\acrodef{PSP}[PSP]{principal state of polarization}

\acrodef{QAM}[QAM]{quadrature amplitude modulation}

\acrodef{RRC}[RRC]{root-raised cosine}

\acrodef{SER}[SER]{symbol error rate}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{sps}[sps]{samples per symbol}

\acrodef{VAE}[VAE]{variational autoencoder}

==> chapters/results_old.tex <==
All numerical results are simulated with a symbol rate of $R_{\mathrm{S}}=\SI{100}{\giga Bd}$, an oversampling of $N_\mathrm{os}=2$~\ac{sps}, and an SNR of $\SI{24}{dB}$ for uniform and $\SI{22}{dB}$ for \ac{PCS}-$64$-QAM with $\mathcal{H}=5.73$. 

First, we analyze the convergence behavior at a challenging working point with $\gammahv=\num{0.2}\pi$, $\taupmd = \frac{T_\mathrm{S}}2 = \frac1{2 R_\mathrm{S}}$, and for various lengths $\Lcd$ of uncompensated fiber as depicted in Fig.~\ref{Results:Lcd_full}. To take the potentially long channel impulse response into account, we use $\Mest=25$~taps. While the \ac{VAE} equalizers achieve the highest \ac{BMI} (dashed lines), the CMAbatch is the most stable algorithm for uniform QAM, where it converges reliably and within 5 frames as depicted in the inlets. The flex schemes converge similarly fast as the CMAbatch but have a higher percentage of failed runs (solid lines) for higher \ac{CD}. However, the VAEflex achieves a significantly higher BMI as the CMAflex. The computationally less expensive VAEbatch converges similarly reliable and equalizes well, as it is indicated by constellation diagram in the right column as well as the high BMI. Its mean frame index of convergence $\bar{k}$ depends on the \ac{CD} and is significantly higher as the flex' ones, but lower as the CMA's $\bar{k}$ for low \ac{CD} or $\Meq=25$. 
The bottom row depicts the results for moderately shaped \ac{PCS}-64-QAM with an entropy of $\mathcal{H}=5.73$, which is commonly-known as challenging task for the \ac{CMA} based state-of-the-art blind equalizers. Only the VAE based equalizers, which consider the \textit{a~priori} density, converge reliably until the \ac{CD} becomes too strong, while the CMAflex fails completely. The VAEflex is still converging within 10 frames but the VAEbatch converges more reliably, especially for $\Meq=25$. 

At $\gammahv=\frac{\pi}4$, the \ac{CMA}'s loss function has a local minimum at an invalid constellation, so the left plot of Fig.~\ref{Results:pol} depicts a sweep of $\gammahv$ around that point. We set a rather strong \ac{PMD} with $\taupmd=T_\mathrm{S}$ and a moderate $\Lcd=\SI{1}{\kilo\meter}$, so we can use $\Meq=\Mest=15$. While the BMI stays similar, the percentage of failed runs increases significantly at $\gammahv\rightarrow\frac{\pi}4$  for all \ac{CMA} based equalizers, which eventually fail in over 50\% of the runs. However, the VAE based equalizers do not struggle at all for this working point. 
The right plot shows the convergence behavior at the critical point of $\gammahv=\frac{\pi}4$. We chose three runs per algorithm representing a good (dash-dotted) and a bad (dotted) performance as well as typical curve (solid) of the converged runs. While the \ac{CMA} based equalizers quickly reach a moderate BMI and converge slowly but gradually, the VAE based algorithms start at low BMI but converge rapidly. Hence, they reach its maximum BMI faster as the CMA based equalizers, including the CMAbatch which reaches $\mathrm{BMI}_\mathrm{thr}=5$ early. The VAE based equalizers have a higher variance than the CMA based ones, where latter either converge similarly or not at all. The curves exhibit that all algorithms are significantly affected by the learning rate scheduler, which might be subject of further optimization. 
